Neural Dynamic Programming for Musical Self Similarity

We present a neural sequence model designed specifically for symbolic music. The model is based on a learned edit distance mechanism which generalises a classic recursion from computer sci- ence, leading to a neural dynamic program. Re- peated motifs are detected by learning the transfor- mations between them. We represent the arising computational dependencies using a novel data structure, the edit tree; this perspective suggests natural approximations which afford the scaling up of our otherwise cubic time algorithm. We demonstrate our model on real and synthetic data; in all cases it out-performs a strong stacked long short-term memory benchmark.

==> figs/raw/Css/2018_02_05_15_21_13_743520_948646797/table_test.tex <==
\motifnettablename & 
1.77 & 1.88 & 0.81 & 1.90 \\ 


